Neuro-BERT: Rethinking Masked Autoencoding for Self-supervised Neurological Pretraining

Deep learning associated with neurological signals is poised to drive major advancements in diverse fields such as medical diagnostics, neurorehabilitation, and brain-computer interfaces. The challenge in harnessing the full potential of these signals lies in the dependency on extensive, high-quality annotated data, which is often scarce and expensive to acquire, requiring specialized infrastructure and domain expertise. To address the appetite for data in deep learning, we present Neuro-BERT, a self-supervised pre-training framework of neurological signals based on masked autoencoding in the Fourier domain. The intuition behind our approach is simple: frequency and phase distribution of neurological signals can reveal intricate neurological activities. We propose a novel pre-training task dubbed Fourier Inversion Prediction (FIP), which randomly masks out a portion of the input signal and then predicts the missing information using the Fourier inversion theorem. Pre-trained models can be potentially used for various downstream tasks such as sleep stage classification and gesture recognition. Unlike contrastive-based methods, which strongly rely on carefully hand-crafted augmentations and siamese structure, our approach works reasonably well with a simple transformer encoder with no augmentation requirements. By evaluating our method on several benchmark datasets, we show that Neuro-BERT improves downstream neurological-related tasks by a large margin.

==> figs/exp_ninapro.tex <==
\begin{table*}[t]
    \setlength{\tabcolsep}{1.2mm}
    \caption{Comparison with previous works for classification and regression tasks on Ninapro DB5 dataset. Acc (\%), mAP (\%), macro F1 (\%), MSE (10$^{-2}$), and MAE (10$^{-2}$) for linear and fine-tuning evaluations are reported.}
    \vspace{-6pt}
    \centering
\resizebox{0.90\linewidth}{!}{
\begin{tabular}{l|cc|cccc|cc} 
\toprule
                                   &                &             & \multicolumn{4}{c|}{Ninapro (Classification)}                                                                     & \multicolumn{2}{c}{Ninapro (Regression)}                            \\
Methods                            & Pre-training   & Backbone    & kNN (Acc)$\uparrow$  & SVM (mAP)$\uparrow$  & FT (Acc)$\uparrow$               & FT (F1)$\uparrow$                & FT(MSE)$\downarrow$             & FT(MAE)$\downarrow$               \\ 
\hline
Rand. init.                        & Random         & ConvNet     & 64.69 $\pm$5.79      & 10.61 $\pm$3.43      & 91.21 $\pm$0.52                  & 80.35 $\pm$0.89                  & 5.61 $\pm$0.54                  & 63.38 $\pm$2.57                   \\
SimAttn~\cite{josephs2020semg}     & Supervised     & ConvNet     & -                    & -                    & 89.15$\pm$0.67                   & 78.96$\pm$0.78                   & 5.73$\pm$0.66                   & 63.32$\pm$2.63                    \\
SimCLR~\cite{chen2020simple}       & Contrastive    & ConvNet     & 87.14 $\pm$0.82      & 65.86 $\pm$0.87      & 91.73 $\pm$0.75                  & 80.86 $\pm$0.67                  & 5.54 $\pm$0.57                  & 63.50 $\pm$1.64                   \\
BYOL~\cite{nips2020byol}           & Contrastive    & ConvNet     & 85.57 $\pm$0.87      & 66.02 $\pm$0.96      & 91.56 $\pm$0.84                  & 80.69 $\pm$0.95                  & 5.72 $\pm$0.45                  & 63.74 $\pm$1.97                   \\
SwAV~\cite{caron2020unsupervised}  & Contrastive    & ConvNet     & 86.13 $\pm$2.33      & 64.43 $\pm$2.12      & 91.84 $\pm$1.76                  & 81.07 $\pm$2.45                  & 5.78 $\pm$0.65                  & 63.32 $\pm$2.20                   \\
MoCo.V3~\cite{chen2021empirical}   & Contrastive    & ConvNet     & 87.45 $\pm$0.66      & 66.29 $\pm$0.78      & 92.14 $\pm$0.66                  & 81.45 $\pm$0.78                  & 5.46 $\pm$0.39                  & 62.83 $\pm$1.92                   \\
TS-TCC~\cite{ijcai2021-324}        & Contrastive    & ConvNet     & 86.87 $\pm$0.95      & 66.10 $\pm$0.93      & 92.02 $\pm$0.95                  & 80.93 $\pm$1.12                  & 5.14 $\pm$0.40                  & 62.95 $\pm$1.83                   \\ 
\hline
Rand. init.                        & Random         & Transformer & 65.28 $\pm$4.73      & 11.07 $\pm$4.51      & 91.97 $\pm$0.58                  & 81.46 $\pm$0.56                  & 5.28 $\pm$0.48                  & 61.21 $\pm$1.93                   \\
MoCo.V3~\cite{chen2021empirical}   & Contrastive    & Transformer & \bf{89.01 $\pm$0.71} & \bf{69.34 $\pm$0.74} & 92.15 $\pm$0.71                  & 83.23 $\pm$0.72                  & 5.57 $\pm$0.51                  & 62.38 $\pm$2.04                   \\ \rowcolor{gray95}
MAE~\cite{he2021masked}            & Autoregressive & Transformer & 77.53 $\pm$0.84      & 48.67 $\pm$0.82      & 93.03 $\pm$0.78                  & 84.32 $\pm$0.82                  & 5.03 $\pm$0.45                  & 60.79 $\pm$1.71                   \\ \rowcolor{gray95}
\bf{neuro2vec}                     & Autoregressive & Transformer & 79.38 $\pm$0.82      & 53.25 $\pm$0.84      & \textbf{94.28}$\pm$\textbf{0.72} & \textbf{86.69}$\pm$\textbf{0.78} & \textbf{4.72}$\pm$\textbf{0.43} & \textbf{60.11}$\pm$\textbf{1.46}  \\
\bottomrule
\end{tabular}
    }
    \vspace{-6pt}
    \label{tab:exp_ninapro}
\end{table*}


==> tabs/tab_sleep_epi.tex <==
\begin{table*}[t]
    \setlength{\tabcolsep}{1.0mm}
    \caption{Comparison with previous self-supervised methods on SleepEDF and Epilepsy datasets. Acc (\%), mAP (\%), and macro F1 (\%) for linear and fine-tuning evaluations are reported.}
    \vspace{-6pt}
    \centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|cc|cccc|cccc} 
\toprule
                                     &                &             & \multicolumn{4}{c|}{SleepEDF}                                                                                   & \multicolumn{4}{c}{Epilepsy}                                                                                     \\
Methods                              & Pre-training   & Backbone    & kNN (Acc)$\uparrow$ & SVM (mAP)$\uparrow$ & FT (Acc)$\uparrow$               & FT (F1)$\uparrow$                & kNN (Acc)$\uparrow$ & SVM (mAP)$\uparrow$ & FT (Acc)$\uparrow$               & FT (F1)$\uparrow$                 \\ 
\hline
Rand. init.                          & Random         & ConvNet     & 65.82$\pm$4.96      & 69.15$\pm$4.14      & 83.34$\pm$0.42                   & 76.71$\pm$0.65                   & 90.13$\pm$3.56      & 97.52$\pm$4.35      & 97.46$\pm$0.26                   & 95.61$\pm$0.42                    \\
AttnSleep~\cite{eldele2021attention} & Supervised     & ConvNet     & -                   & -                   & 84.23$\pm$0.56                   & 77.84$\pm$0.74                   & -                   & -                   & 97.35$\pm$0.31                   & 94.54$\pm$0.57                    \\
SimCLR~\cite{chen2020simple}         & Contrastive    & ConvNet     & 72.47$\pm$0.84      & 75.47$\pm$0.68      & 83.60$\pm$0.79                   & 76.96$\pm$0.89                   & 95.28$\pm$0.56      & 96.09$\pm$0.64      & 97.52$\pm$0.41                   & 95.98$\pm$0.76                    \\
BYOL~\cite{nips2020byol}             & Contrastive    & ConvNet     & 71.65$\pm$0.73      & 75.26$\pm$0.81      & 83.29$\pm$0.76                   & 76.68$\pm$0.94                   & 94.54$\pm$0.48      & 96.64$\pm$0.52      & 97.94$\pm$0.64                   & 96.70$\pm$0.87                    \\
SwAV~\cite{caron2020unsupervised}    & Contrastive    & ConvNet     & \bf{76.19$\pm$1.24} & 76.83$\pm$1.56      & 83.84$\pm$1.35                   & 77.18$\pm$1.62                   & 95.95$\pm$1.23      & 98.36$\pm$1.43      & 98.60$\pm$1.12                   & 97.82$\pm$0.53                    \\
MoCo.V3~\cite{chen2021empirical}     & Contrastive    & ConvNet     & 72.53$\pm$0.75      & 75.51$\pm$0.84      & 83.46$\pm$0.68                   & 76.70$\pm$0.76                   & 94.33$\pm$0.31      & 95.09$\pm$0.34      & 98.74$\pm$0.58                   & 97.98$\pm$0.64                    \\
TS-TCC~\cite{ijcai2021-324}          & Contrastive    & ConvNet     & 73.87$\pm$0.76      & 76.12$\pm$0.98      & 84.05$\pm$0.82                   & 77.04$\pm$0.88                   & 96.98$\pm$0.35      & 98.74$\pm$0.37      & 98.75$\pm$0.78                   & 97.81$\pm$0.72                    \\ 
\hline
Rand. init.                          &Random          & Transformer & 66.75$\pm$4.10      & 69.50$\pm$3.26      & 84.20$\pm$0.41                   & 77.15$\pm$0.59                   & 90.23$\pm$3.74      & 96.29$\pm$4.03      & 97.88$\pm$0.27                   & 96.54$\pm$0.38                    \\
MoCo.V3~\cite{chen2021empirical}     & Contrastive    & Transformer & 75.61$\pm$0.63      & \bf{77.84$\pm$0.82} & 85.49$\pm$0.72                   & 77.73$\pm$0.80                   & \bf{98.17$\pm$0.34} & \bf{98.91$\pm$0.42} & 98.93$\pm$0.59                   & 98.60$\pm$0.58                    \\ \rowcolor{gray95}
MAE~\cite{he2021masked}              & Autoregressive & Transformer & 68.43$\pm$0.89      & 70.78$\pm$0.94      & 85.08$\pm$0.89                   & 77.40$\pm$0.86                   & 90.64$\pm$0.49      & 96.95$\pm$0.59      & 99.15$\pm$0.74                   & 98.79$\pm$0.64                    \\ \rowcolor{gray95}
\bf{neuro2vec}                       & Autoregressive & Transformer & 69.55$\pm$0.82      & 71.49$\pm$0.84      & \textbf{86.53}$\pm$\textbf{0.83} & \textbf{78.94}$\pm$\textbf{0.87} & 93.78$\pm$0.47      & 97.06$\pm$0.57      & \textbf{99.34}$\pm$\textbf{0.66} & \textbf{98.82}$\pm$\textbf{0.65}  \\
\bottomrule
\end{tabular}
    }
    \label{tab:exp_sleep_epi}
    \vspace{-6pt}
\end{table*}

